LeNSE: Learning To Navigate Subgraph Embeddings for Large-Scale Combinatorial Optimisation

Combinatorial Optimisation problems arise in several application domains and are often formulated in terms of graphs. Many of these problems are NP-hard, but exact solutions are not always needed. Several heuristics have been developed to provide near-optimal solutions; however, they do not typically scale well with the size of the graph. We propose a low-complexity approach for identifying a (possibly much smaller) subgraph of the original graph where the heuristics can be run in reasonable time and with a high likelihood of finding a global near-optimal solution. The core component of our approach is LeNSE, a reinforcement learning algorithm that learns how to navigate the space of possible subgraphs using an Euclidean subgraph embedding as its map. To solve CO problems, LeNSE is provided with a discriminative embedding trained using any existing heuristics using only on a small portion of the original graph. When tested on three problems (vertex cover, max-cut and influence maximisation) using real graphs with up to $10$ million edges, LeNSE identifies small subgraphs yielding solutions comparable to those found by running the heuristics on the entire graph, but at a fraction of the total run time.

==> preamble.tex <==
%---------------------------------------------------------%
%------------------ Document Preamble --------------------%
%---------------------------------------------------------%

%-------------------------------------------%
%---- First load the necessary packages ----%
%-------------------------------------------%

\usepackage{graphicx} % For including graphics (via \includegraphics).
\usepackage{amsmath}  % Improves typographic quality of mathematical output.
\usepackage{amsfonts} % For mathematical fonts.
% \usepackage{amssymb}

% Set the layout of the document.
\usepackage{xcolor}
\usepackage{framed} %for shading parts of document
\usepackage{lipsum}
\usepackage{color,soul} %for highlighting
\usepackage[scale=0.7,vmarginratio={1:2},heightrounded]{geometry}
\usepackage{amsthm} % Needed to typeset theorem environments.
\usepackage[affil-it]{authblk} % Needed for author and affiliation.
\usepackage{amsopn} % Allows the declaration of new mathematical operators.
\usepackage{amssymb} % Extended set of mathematical symbols.
\usepackage{mathrsfs} % Raph Smith's mathematical script font.
\usepackage{booktabs} % Improves the typographical quality of tables.
% \usepackage{cite}
% \usepackage{natbib}
\usepackage{tikz} % Extends the figure generation capabilities of LaTeX.
\usepackage{algorithm} % Necessary for including algorithmic structures.
\usepackage{float} % Allows the creation of own floating environments.
\usepackage{caption} % Allows the customisation of captions.
\usepackage{abstract} % For including abstracts in documents.
\usepackage{listings} % For the inclusion of source code.
\usepackage{color} % Used for colour commands.
\usepackage{pgfplots} %more complex graphs


% % Automatic inclusion of hyperlinks with back references.
\usepackage[pagebackref]{hyperref} 

%-------------------------------------------%

% Making a float for an algorithm.
\newfloat{algorithm}{t}{lop}
\renewcommand{\thealgorithm}{\arabic{section}.\arabic{algorithm}} 

% Numbers equations by section.
\numberwithin{equation}{section}

% % Set biliography style.
% \bibliographystyle{abbrv}

% Commands for special set of numbers.
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\CC}{\mathbb{C}}

% Commands for useful operators.
\newcommand{\di}{\text{diag}}
\newcommand{\de}{\mathrm{d}}
\newcommand{\si}{\Sigma}
\newcommand{\del}{\Delta}
\newcommand{\cov}[1]{\, {\rm cov}\left( #1 \right) }
\newcommand{\var}[1]{\, {\rm var}\left( #1 \right) }
\newcommand{\toas}{\xrightarrow{\text{a.s.}}}
\newcommand{\todis}{\xrightarrow{\text{d}}}
\newcommand{\supp}{\text{supp}}
\newcommand{\doubint}{\!\int\!\!\!\int}

% Command for text within a math sub/super-script.
\newcommand{\stext}[1]{\text{\scriptsize{#1}}}

% % Theorem definitions/
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{theorem}[lemma]{Theorem}
% \newtheorem{proposition}[lemma]{Proposition}
% \newtheorem{corollary}[lemma]{Corollary}

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]

% \theoremstyle{remark}
% \newtheorem{remark}{Remark}[section]
% \newtheorem{example}[remark]{Example}

% An environment for centre aligning equations which extend past the text width.
\newenvironment{longeq}
 {\begin{displaymath}\begin{lrbox}{\overlongequation}$\displaystyle}
 {$\end{lrbox}\makebox[0pt]{\usebox{\overlongequation}}\end{displaymath}}

% Listings options.

\lstset{ %
basicstyle=\footnotesize,       % the size of the fonts that are used for the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=false,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}

